Z-LaVI: Zero-Shot Language Solver Fueled by Visual Imagination

Large-scale pretrained language models have made significant advances in solving downstream language understanding tasks. However, they generally suffer from reporting bias, the phenomenon describing the lack of explicit commonsense knowledge in written text, e.g., ''an orange is orange''. To overcome this limitation, we develop a novel approach, Z-LaVI, to endow language models with visual imagination capabilities. Specifically, we leverage two complementary types of ''imaginations'': (i) recalling existing images through retrieval and (ii) synthesizing nonexistent images via text-to-image generation. Jointly exploiting the language inputs and the imagination, a pretrained vision-language model (e.g., CLIP) eventually composes a zero-shot solution to the original language tasks. Notably, fueling language models with imagination can effectively leverage visual knowledge to solve plain language tasks. In consequence, Z-LaVI consistently improves the zero-shot performance of existing language models across a diverse set of language tasks.

==> [EMNLP 2022] Z-LaVI/tables/clip_text_only.tex <==
\begin{table}[!t]
\centering
\resizebox{7.7cm}{!}{
\begin{tabular}{ccccccc}
\Xhline{3\arrayrulewidth}
 & \textbf{QASC} & \textbf{SciQ} & \textbf{ARC} & \textbf{WSD} & \textbf{AG} & \textbf{Situ} \\ \hline
\# TOK   &  2.4    & 2.6    & 4.9 & 28.4  &  54.7  &  56.8    \\ \hline
\xmark  &  26.8    & 41.1    & 42.1 & 75.0  &  52.9  &  22.4    \\
\textsc{Recall}    &  \underline{32.6}    & \textbf{49.9}     &   \underline{48.5} & 80.3  & 52.5   &  21.1  \\
\textsc{Synthesis}  & 31.5 & 39.9 & 44.6 & \underline{81.5} & \textbf{71.6} & \textbf{34.2}\\
\textsc{Both}  & \textbf{32.7} & \underline{49.5} & \textbf{50.2} & \textbf{83.8} & \textbf{71.6} & \underline{33.4} \\\Xhline{3\arrayrulewidth}
 
\end{tabular}
}
\caption{The performance of Z-LaVI (w/o LM) with different imagination methods. \# TOK is the average number of tokens of text inputs in each dataset. \xmark~means no image is provided to the model, and we only use the text encoder of CLIP. \textsc{Recall} and \textsc{Synthesis} represent using image search and image generation, respectively. \textsc{Both} means combining the two methods.}
\label{tab image method}
\end{table}


==> [EMNLP 2022] Z-LaVI/tables/dataset_stat.tex <==
\begin{table}[!t]
\centering
\resizebox{7.7cm}{!}{
\begin{tabular}{cccc}
\Xhline{3\arrayrulewidth}  
\textbf{Task}    & \textbf{Dataset}     & \textbf{Split} & \textbf{\# samples} \\ \hline
WSD & CoarseWSD-20 & test  &  10,196\\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Science \\QA\end{tabular}} & QASC        & dev   & 926        \\
                            & SciQ        & dev   & 1,000      \\
                            & ARC-E       & dev   & 570        \\
                            & ARC-C       & dev   & 299        \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Text \\  Classification\end{tabular}} & AG-News     & test  & 7,600      \\
                            & Situation   & test  & 1,789     \\\Xhline{3\arrayrulewidth}  
\end{tabular}
}
\caption{Dataset statistics for the three tasks.}
\label{tab: data stat}
\end{table}

==> [EMNLP 2022] Z-LaVI/tables/model_size.tex <==
% \begin{table*}[!t]
% \centering
% \small
% \begin{tabular}{ccccccccc}
% \Xhline{3\arrayrulewidth}  
% \textbf{Model}         & \textbf{CLIP} & \textbf{BART-L} & \textbf{RoBERTa-L} & \textbf{SBERT} & \textbf{SimCSE} & \textbf{GPT-Neo-1.3B} & \textbf{GPT-Neo-2.7B} & \textbf{GPT-J} \\ \hline
% \# parameters & 150M & 400M   & 355M    & 110M  & 355M   & 1.3B   & 2.7B      & 6B    \\
% $w$             & -    & 0.59  & 0.6     & 0.80  & 0.60   & 0.53   & 0.51      & 0.51 \\\Xhline{3\arrayrulewidth}  
% \end{tabular}
% \caption{The number of parameters of each model and the ensemble weights calculated by equation \ref{eq: ensemble weight}.}
% \label{tab n parameters}
% \end{table*}

\begin{table}[!htbp]
\centering
\small
\begin{tabular}{ccc}
\Xhline{3\arrayrulewidth}      
\textbf{Model}        & \textbf{\# of Parameters} & \textbf{Ensemble weight} \\ \hline
CLIP         & 150 M            & -               \\
BART-L       & 400 M            & 0.59            \\
RoBERTa-L    & 355 M            & 0.60            \\
SBERT        & 110 M            & 0.80            \\
SimCSE       & 355 M            & 0.60            \\
GPT-Neo-1.3B & 1.3 B            & 0.53            \\
GPT-Neo-2.7B & 2.7 B            & 0.51            \\
GPT-J-6B     & 6 B              & 0.51            \\
OPT-30B      & 30 B             & 0.50            
\\\Xhline{3\arrayrulewidth}      
\end{tabular}
\caption{The number of parameters of each model and the ensemble weights calculated by equation \ref{eq: ensemble weight}.}
\label{tab n parameters}
\end{table}

==> [EMNLP 2022] Z-LaVI/tables/prompt.tex <==
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{cccc}
\Xhline{3\arrayrulewidth}  
\textbf{Model} & \textbf{Word Sense Disambiguation} & \textbf{Question Answering} & \textbf{Topic Classification} \\ \hline
\begin{tabular}[c]{@{}c@{}}GPT\\ NLI\end{tabular} & \begin{tabular}[c]{@{}c@{}}{[}SENTENCE{]} The {[}TARGET WORD{]} \\ mentioned before means {[}SENSE NAME{]}.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Question: {[}QUESTION{]} \\ The answer is {[}ANSWER{]}.\end{tabular} & \begin{tabular}[c]{@{}c@{}}{[}SENTENCE{]} This example \\ is {[}CLASS NAME{]}.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}SimCSE\\ SBERT\end{tabular}   & (SENTENCE, DEFINITION)   & (QUESTION, ANSWER) & \begin{tabular}[c]{@{}c@{}}(SENTENCE, This example \\ is {[}CLASS NAME{]}.)\end{tabular}    \\ \hline
CLIP    & (SENTENCE, DEFINITION)     & (QUESTION, ANSWER) & \begin{tabular}[c]{@{}c@{}}(SENTENCE, A news image \\ of {[}CLASS NAME{]}.)\end{tabular}   \\\Xhline{3\arrayrulewidth}  
\end{tabular}
\caption{The prompts we use for each model on WSD, QA, and Topic classification.}
\label{tab: prompt}
\end{table*}

==> [EMNLP 2022] Z-LaVI/tables/qa.tex <==
% \begin{table*}[!t]
% \centering
% \small
% \resizebox{15cm}{!}{%
% \begin{tabular}{lcccccccc}
% \\\Xhline{2\arrayrulewidth}    
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{QASC}} & \multicolumn{2}{c}{\textbf{SciQ}} & \multicolumn{2}{c}{\textbf{ARC-E}} & \multicolumn{2}{c}{\textbf{ARC-C}} \\ \cline{2-9} 
% & Original  & \model      & Original      & \model      & Original       & \model      & Original      & \model      \\ \hline
% Random       & 12.5    &  -   &  25.0   &  -  &    25.0  & -  & 25.0    & -\\
% IR Solver$^{\dagger}$ &  18.6   &  -  &  -    &  -  &  30.4    & -  &  20.3   & - \\
% SMLM$^{\dagger}$ &  26.6   & - &  -   & - &   33.4   & - &  28.4   & - \\ 
% RoBERTa-L-mnli*   & 19.3   & \underline{26.5}    &  44.7 & \underline{51.7}  &  48.4  & \underline{50.2} &  34.4  & 32.4\\
% BART-L-mnli*   & 21.7    & \underline{26.3}    &  48.8   &  \underline{54.2}   & 54.7     & \underline{56.5} &  \textbf{36.5}   & 34.1\\
% % T5-3B*        &  23.1   & \underline{30.2}    & 41.1    &   &   38.2   &   & 27.4    & \\
% GPT-Neo-1.3B        & 29.3    & \underline{35.2}    &  57.5   & \underline{61.3} &  48.6    &  \underline{51.4} & 26.1     & \underline{26.8}\\
% GPT-Neo-2.7B        & 29.6    & \underline{38.3}    &  64.0   & \underline{65.1}    &   52.1   &  \underline{52.3}   &  30.4    & 27.4\\
% GPT-J-6B        &  36.3   & \underline{39.3}    &  73.2   & \textbf{\underline{73.8}}  &  \textbf{57.7}    & 56.0 & 33.1   & 30.1 \\
% SimCSE       & 30.8    &  \underline{33.8}   &  42.6   & \underline{49.9}  &  43.3    & \underline{47.0}  &  26.4   & 25.8 \\
% SBERT*       &  36.7   & \underline{\textbf{39.8}}    &  57.7   & 57.3    & 52.8     & 54.0 &    30.1 & 26.4\\\hline
% \model~w/o LM    &  -   & 31.3   &  -   &  51.0   &  -    & 44.6 &   -  &  25.8 \\\Xhline{2\arrayrulewidth}    
% \end{tabular}
% }
% \caption{Zero-shot performance on Science QA tasks. \model~represents the performance with our Visual Imagination. \model~(w/o LM) is the model only uses vision-text prediction. The best-performed number for each metric is \textbf{bolded}. The numbers are \underline{underlined} if the original performance is improved with \model. * indicates the model uses labeled data for pre-training. The model with $\dagger$ means the results are from previous work.}
% \label{tab: qa}
% \end{table*}

\begin{table*}[!t]
\centering
\small
% \resizebox{15cm}{!}{%
\begin{tabular}{lccccccccc}
\\\Xhline{2\arrayrulewidth}    
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\# Param.}} & \multicolumn{2}{c}{\textbf{QASC}} & \multicolumn{2}{c}{\textbf{SciQ}} & \multicolumn{2}{c}{\textbf{ARC-E}} & \multicolumn{2}{c}{\textbf{ARC-C}} \\ \cline{3-10} 
& & Original  & \model      & Original      & \model      & Original       & \model      & Original      & \model      \\ \hline
Random       & - & 12.5    &  -   &  25.0   &  -  &    25.0  & -  & 25.0    & -\\
IR Solver$^{\dagger}$ & - &  18.6   &  -  &  -    &  -  &  30.4    & -  &  20.3   & - \\
SMLM$^{\dagger}$ & 355 M &  26.6   & - &  -   & - &   33.4   & - &  28.4   & - \\ 
RoBERTa-L-mnli*  & 355 M & 19.3   & \underline{27.2}    &  44.7 & \underline{51.3}  &  48.4  & \underline{51.8} &  34.4  & 33.4\\
BART-L-mnli*   & 400 M & 21.7    & \underline{27.3}    &  48.8   &  \underline{51.0}   & 54.7     & \underline{56.1} &  \textbf{36.5}   & \textbf{36.5}\\
GPT-Neo-1.3B    &  1.3B   & 29.3    & \underline{37.4}    &  57.5   & \underline{60.8} &  46.3 & \underline{49.8} & 27.4 & 26.1\\
GPT-Neo-2.7B    &  2.7B   & 29.6    & \underline{39.6}    &  64.0   & \underline{64.9}    &  49.6   &  \underline{51.9}   &  31.8    & 30.4\\
GPT-J-6B     &  6B  &  36.3   & \underline{42.0}    &  73.2   & \underline{73.7} &  55.1    & \underline{57.2} & 34.8   & 34.1 \\
OPT-30B & 30B & 39.7 & \underline{\textbf{42.1}} & 72.7 & \underline{\textbf{74.0}} & 58.2 & \underline{\textbf{59.5}} & 34.8 & 34.1\\
SimCSE     & 355M  & 30.8    &  \underline{33.2}   &  42.6   & \underline{48.6}  &  43.3    & \underline{49.3}  &  26.4   & 24.7 \\
SBERT*     & 110M  &  36.7   & \underline{38.6}    &  57.7   & \underline{58.5}    & 54.4     & \underline{56.0} &    30.1 & 27.1\\\hline
\model~w/o LM  & 150M  &  -   & 32.7   &  -   &  49.5   &  -    & 50.2 &   -  &  26.7 \\\Xhline{2\arrayrulewidth}    
\end{tabular}
% }
\caption{Zero-shot performance on Science QA tasks. \model~represents the performance with our Visual Imagination. \model~(w/o LM) is the model that only uses vision-text prediction. The best-performed number for each metric is \textbf{bolded}. The numbers are \underline{underlined} if the original performance is improved with \model. The models with * use labeled data for pre-training. The models with $\dagger$ indicate the results are from previous work.}
\label{tab: qa}
\end{table*}

==> [EMNLP 2022] Z-LaVI/tables/tc.tex <==
\begin{table}[!t]
\centering
\resizebox{7.7cm}{!}{
\begin{tabular}{lcccc}
\Xhline{3\arrayrulewidth}  
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{AG-News}} & \multicolumn{2}{c}{\textbf{Situation}} \\ \cline{2-5} 
    & Orig.  & \model    & Orig. & \model  \\ \hline
Random       &   25.0  &   -   &    9.1   &    -   \\
TE-wiki$^{\dagger}$*     &   79.6  &   -   &     -    &    -   \\
RoBERTa-L-mnli*  &   81.2  &  \underline{81.7}     &  40.7  &  \underline{41.8}  \\
BART-L-mnli*  &   81.9  &  \underline{\textbf{82.4}}     &  40.5  &  \underline{41.1}  \\
% T5-3B*       &   62.6  &       &     &    \\
GPT-Neo-1.3B &   59.1  &  \underline{72.9}     & 17.8     & \underline{38.5}   \\
GPT-Neo-2.7B &   59.1  &  \underline{74.5}     &  13.6   &   \underline{35.2} \\
GPT-J-6B     &   61.0  &   \underline{73.8}    &  21.9   &  \underline{38.8}  \\
% OPT-30B \\
SimCSE       &   58.1  &  \underline{73.1}     &  42.1   &  \underline{44.4}  \\
SBERT*       &   77.8  &  \underline{82.2}     & 42.6    &  \underline{\textbf{46.6}}     \\ \hline
\model~w/o LM       &    -     &  71.6     &  -   &  33.4  \\ \Xhline{3\arrayrulewidth}
\end{tabular}
}
\caption{Zero-shot Performance on Topic Classification.}
\label{tab: tc}
\end{table}
\vspace{-.2cm}


==> [EMNLP 2022] Z-LaVI/tables/vicomte.tex <==
% \begin{table*}[]
% \centering
% \resizebox{16cm}{!}{%
% \begin{tabular}{lcccc|cccc|cccc}
% \Xhline{3\arrayrulewidth}  
% \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{\textsc{Color}}} & \multicolumn{4}{c|}{\textbf{\textsc{Shape}}} & \multicolumn{4}{c}{\textbf{\textsc{Material}}} \\ \cline{2-13}
% & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{Z-LaVI} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{Z-LaVI} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Z-LaVI} \\
% & Spears $\rho$ & Acc@1 & Spears $\rho$ & Acc@1 & Spears $\rho$ & Acc@1 & Spears $\rho$ & Acc@1 & Spears $\rho$ & Acc@1 & Spears $\rho$ & Acc@1 \\\hline

% BERT-L$^{\dagger}$  & 37.6$_{\pm30.3}$ & 30.3 & - & - & 42.7$_{\pm17.1}$ & 28.4 & - & - & 36.6$_{\pm19.1}$ & 35.7 & - & - \\
% Oscar-L$^{\dagger}$ & 31.8$_{\pm28.3}$ & 17.1 & - & - & 40.0$_{\pm16.9}$ & 38.1 & - & - & \textbf{39.2$_{\pm17.1}$} & 40.5 & - & - \\

% GPT-Neo-1.3B & 40.1$_{\pm26.5}$ & 31.7 & \underline{47.4$_{\pm23.0}$} & \underline{48.4} & 44.2$_{\pm15.6}$ & 52.9 & \underline{46.1$_{\pm15.1}$} & \underline{64.3} & 35.1$_{\pm18.0}$ & 34.5 & \underline{36.4$_{\pm17.8}$} & \underline{41.2} \\
% GPT-Neo-2.7B & 41.3$_{\pm26.9}$ & 29.3 & \underline{47.0$_{\pm24.5}$} & \underline{43.6} & 43.4$_{\pm18.0}$ & 49.3 & \underline{45.1$_{\pm16.7}$} & \underline{62.1} & 35.5$_{\pm18.6}$ & 30.6 & \underline{36.1$_{\pm18.6}$} & \underline{37.7}\\
% GPT-J-6B     & 44.3$_{\pm25.7}$ & 38.0 & \underline{\textbf{49.6$_{\pm23.7}$}} & \underline{\textbf{50.9}} & 46.6$_{\pm16.2}$ & 64.3 & \underline{\textbf{46.8$_{\pm23.7}$}} & \underline{\textbf{68.6}} & 38.5$_{\pm17.7}$ & 42.3 & 37.9$_{\pm18.8}$ & \underline{\textbf{46.5}}\\
% Z-LaVI w/o LM & - & - & 37.2$_{\pm25.7}$ & 39.4 & - & - & 33.8$_{\pm20.3}$ & 32.1 & - & - & 24.9$_{\pm21.9}$ & 32.7 \\ \Xhline{3\arrayrulewidth}
% \end{tabular}
% }
% \caption{Zero-shot Probing on the three groups of relations in ViComTe dataset. We report the average Spearman correlation (Spears. $\rho$) and top-1 accuracy (Acc@1).}
% \end{table*}

% \begin{table*}[!t]
% \centering
% \resizebox{16cm}{!}{%
% \begin{tabular}{lcccc|cccc|cccc|cc}
% \Xhline{3\arrayrulewidth}  
% \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{\textsc{Color}}} & \multicolumn{4}{c|}{\textbf{\textsc{Shape}}} & \multicolumn{4}{c|}{\textbf{\textsc{Material}}} & \multicolumn{2}{c}{\textbf{\textsc{Cooccur}}} \\ \cline{2-15}
% & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{Z-LaVI} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{Z-LaVI} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{Z-LaVI} & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{Z-LaVI}\\
% & $\rho$ & Acc@1 & $\rho$ & Acc@1 &  $\rho$ & Acc@1 &  $\rho$ & Acc@1 &  $\rho$ & Acc@1 &  $\rho$ & Acc@1 &  $\rho$ &  $\rho$\\\hline

% BERT-L$^{\dagger}$  & 37.6 & 30.3 & - & - & 42.7 & 28.4 & - & - & 36.6 & 35.7 & - & - & 5.2 & -\\
% Oscar-L$^{\dagger}$ & 31.8 & 17.1 & - & - & 40.0 & 38.1 & - & - & \textbf{39.2} & 40.5 & - & - & 9.7 & - \\

% GPT-Neo-1.3B & 40.1 & 31.7 & \underline{47.4} & \underline{48.4} & 44.2 & 52.9 & \underline{46.1} & \underline{64.3} & 35.1 & 34.5 & \underline{36.4} & \underline{41.2} \\
% GPT-Neo-2.7B & 41.3 & 29.3 & \underline{47.0} & \underline{43.6} & 43.4 & 49.3 & \underline{45.1} & \underline{62.1} & 35.5 & 30.6 & \underline{36.1} & \underline{37.7}\\
% GPT-J-6B     & 44.3 & 38.0 & \underline{\textbf{49.6}} & \underline{\textbf{50.9}} & 46.6 & 64.3 & \underline{\textbf{47.0}} & \underline{\textbf{68.6}} & 38.5 & 42.3 & 37.9 & \underline{\textbf{46.5}}\\
% Z-LaVI w/o LM & - & - & 37.2 & 39.4 & - & - & 33.8 & 32.1 & - & - & 24.9 & 32.7 & - & 4.0 \\ \Xhline{3\arrayrulewidth}
% \end{tabular}
% }
% \caption{Zero-shot probing on the three relation groups in ViComTe dataset. We report the average Spearman correlation ($\rho$) and top-1 accuracy (Acc@1).}
% \label{tab: vicomte}
% \end{table*}

\begin{table*}[!t]
\centering
\resizebox{16cm}{!}{%
\begin{tabular}{lcccc|cccc|cccc}
\Xhline{3\arrayrulewidth}  
\multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{\textsc{Color}}} & \multicolumn{4}{c|}{\textbf{\textsc{Shape}}} & \multicolumn{4}{c}{\textbf{\textsc{Material}}}\\ \cline{2-13}
& \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{Z-LaVI} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{Z-LaVI} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Z-LaVI} \\
& $\rho$ & Acc@1 & $\rho$ & Acc@1 &  $\rho$ & Acc@1 &  $\rho$ & Acc@1 &  $\rho$ & Acc@1 &  $\rho$ & Acc@1 \\\hline
Random & -0.1 & 6.6 & - & - & 1.3 & 7.1 & - & - & -1.5 & 6.0 & - & -\\
BERT-L$^{\dagger}$  & 37.6 & 30.3 & - & - & 42.7 & 28.4 & - & - & 36.6 & 35.7 & - & - \\
Oscar-L$^{\dagger}$ & 31.8 & 17.1 & - & - & 40.0 & 38.1 & - & - & \textbf{39.2} & 40.5 & - & - \\
RoBERTa-L-mnli* & 35.3 & 25.1 & \underline{41.4} & \underline{38.2} & 41.7 & 66.4 & \underline{43.5} & \underline{67.9} & 28.3 & 34.9 & \underline{31.6} & \underline{37.7} \\
BART-L-mnli* & 34.6 & 27.5 & \underline{38.2} & \underline{32.6} & 41.5 & 68.6 & \underline{42.0} & \underline{69.3} & 30.5 & 37.0 & \underline{32.6} & \underline{40.5}\\
GPT-Neo-1.3B & 40.1 & 31.7 & \underline{47.4} & \underline{48.4} & 44.2 & 52.9 & \underline{46.1} & \underline{64.3} & 35.1 & 34.5 & \underline{36.4} & \underline{41.2} \\
GPT-Neo-2.7B & 41.3 & 29.3 & \underline{47.0} & \underline{43.6} & 43.5 & 50.0 & \underline{45.2} & \underline{62.1} & 35.5 & 30.6 & \underline{36.1} & \underline{37.7}\\
GPT-J-6B     & 44.3 & 38.0 & \underline{\textbf{49.6}} & \underline{50.9} & 46.9 & 65.7 & \underline{47.1} & \underline{70.0} & 38.5 & 42.3 & 37.9 & \underline{46.5}\\
OPT-30B & 41.9 & 41.3 & \underline{48.1} & \underline{\textbf{52.1}} & 46.4 & 60.0 & \underline{\textbf{48.4}} & \underline{\textbf{72.1}} & 38.3 & 44.7 & 38.1 & \underline{\textbf{47.5}}\\
SimCSE & 30.7 & 34.8 & \underline{36.3} & \underline{40.4} & 30.1 & 28.6 & \underline{34.7} & \underline{40.7} & 24.6 & 26.4 & \underline{29.2} & \underline{33.5}\\
SBERT* & 27.6 & 26.5 & \underline{38.2} & \underline{40.6} & 20.3 & 13.6 & \underline{33.6} & \underline{35.0} & 24.1 & 22.5 & \underline{30.4} & \underline{34.9}\\ \hline
Z-LaVI w/o LM & - & - & 37.2 & 39.4 & - & - & 33.8 & 32.1 & - & - & 24.9 & 32.7 \\ \Xhline{3\arrayrulewidth}
\end{tabular}
}
\caption{Zero-shot probing on the three relation types (\textsc{Color}, \textsc{Shape} and \textsc{Material}) in ViComTe \cite{zhang-etal-2022-visual} dataset. We report the average Spearman correlation ($\rho$) and top-1 accuracy (Acc@1).}
\label{tab: vicomte}
\end{table*}

==> [EMNLP 2022] Z-LaVI/tables/vicomte_ablation.tex <==
\begin{table}[!htbp]
\centering
\resizebox{7.5cm}{!}{%
\begin{tabular}{lcccc}
\Xhline{3\arrayrulewidth}  
  $\rho$/Acc@1       & \textbf{\textsc{Recall}} & \textbf{\textsc{Synthesis}} & \textbf{\textsc{Both}} \\ \hline
\textsc{color}       &  35.5/35.7     &   \underline{36.4}/\underline{38.5}    &     \textbf{37.2}/\textbf{39.4}             \\
\textsc{shape}       &  \textbf{37.1}/\textbf{49.3}     &   27.9/31.3    &     \underline{33.9}/\underline{32.1}             \\
\textsc{material}    & \textbf{29.9}/\textbf{34.9}      &   23.4/29.6    &  \underline{24.9}/\underline{32.7}     \\\Xhline{3\arrayrulewidth}  
\end{tabular}
}
\caption{The average Spearman correlation (left) and top-1 accuracy (right) of \model~w/o LM with different imagination methods. The highest number of each row is \textbf{bolded} and the second-best one is \underline{underlined}.}
\label{tab: vicomte ablate}
\end{table}

==> [EMNLP 2022] Z-LaVI/tables/vicomte_prompt.tex <==
\begin{table*}[!htbp]
\centering
\small
\begin{tabular}{ccc}
\Xhline{3\arrayrulewidth}
\textbf{\textsc{Color}} & \textbf{\textsc{Material}} & \textbf{\textsc{Shape}}  \\ \hline
\begin{tabular}[c]{@{}c@{}}{[}SUBJ{]} can be of color {[}OBJ{]}.\\ {[}SUBJ{]} has color {[}OBJ{]}.\\ The color of {[}SUBJ{]} can be {[}OBJ{]}.\\ The color of the {[}SUBJ{]} is {[}OBJ{]}.\\ {[}SUBJ{]} is {[}OBJ{]}.\\ This {[}SUBJ{]} is {[}OBJ{]}.\\ {[}SUBJ{]} is of color {[}OBJ{]}.\end{tabular} & \begin{tabular}[c]{@{}c@{}}{[}SUBJ{]} is made of {[}OBJ{]}.\\ {[}SUBJ{]} can be made of {[}OBJ{]}.\\ {[}SUBJ{]} is made from {[}OBJ{]}.\\ {[}SUBJ{]} can be made from {[}OBJ{]}. \\ {[}SUBJ{]} is {[}OBJ{]}.\\ This {[}SUBJ{]} is {[}OBJ{]}.\\ {[}SUBJ{]} is made by using {[}OBJ{]}.\end{tabular} & \begin{tabular}[c]{@{}c@{}}{[}SUBJ{]} can be shape of {[}OBJ{]}.\\ {[}SUBJ{]} has shape of {[}OBJ{]}.\\ {[}SUBJ{]} is of shape {[}OBJ{]}.\\ The shape of {[}SUBJ{]} can be {[}OBJ{]}.\\ The shape of the {[}SUBJ{]} is {[}OBJ{]}.\\ {[}SUBJ{]} is {[}OBJ{]}.\\ This {[}SUBJ{]} is {[}OBJ{]}.\end{tabular} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{The prompts we use for ViComTe which are provided by \citet{zhang-etal-2022-visual}.}
\end{table*}

==> [EMNLP 2022] Z-LaVI/tables/vicomte_stat.tex <==
\begin{table}[!t]
\centering
\centering
\resizebox{7.7cm}{!}{%
\begin{tabular}{lccc}
\Xhline{3\arrayrulewidth}  
\textbf{Relation}      &    \textbf{\# Objs} & \textbf{\# Test Subjs} & \textbf{Ex (subj, obj) pair}  \\ \hline
\textsc{Color}         &    12 & 574 &  (leave, green)                        \\
\textsc{Shape}         &    12 & 140 &  (egg, oval)                           \\
\textsc{Material}      &    18 & 284 &  (mug, glass)                          \\ \Xhline{3\arrayrulewidth}  
% \textsc{Cooccur}       &    5,939 & 420 &  (ivory, elephant)                   \\ 
\end{tabular}
}
\caption{Statistics of ViComTe dataset.}
\label{tab: vicomte stat}
\vspace{-.2cm}
\end{table}

==> [EMNLP 2022] Z-LaVI/tables/wsd.tex <==
% \begin{table}[!t]
% \centering
% \resizebox{7.7cm}{!}{%
% \begin{tabular}{lcccc}
% \Xhline{3\arrayrulewidth}  
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Accuracy}}             & \multicolumn{2}{c}{\textbf{F1}}       \\ \cline{2-5}
%   & \multicolumn{1}{l}{Orig.} & \multicolumn{1}{l}{\model} & \multicolumn{1}{l}{Orig.} & \multicolumn{1}{l}{\model} \\ \hline
% Random                &   41.3    &   -   &  36.7    &   -   \\
% BERT-L-1shot$^{\dagger}$*          &  77.6    &  -    &  71.2    &   -   \\
% BERT-L-3shot$^{\dagger}$*          &  89.3    &  -    &  85.2    &   -   \\ 
% RoBERTa-L-mnli*           &  80.4    &   \underline{83.0}  & 74.4    &  \underline{78.1}   \\
% BART-L-mnli*           &  80.2    &  \underline{82.2}    &  74.8   &  \underline{77.8}    \\
% GPT-Neo-1.3B          &  74.4    &  \underline{87.9}    &  68.4    & \underline{82.6}    \\
% GPT-Neo-2.7B          &  76.2    &  \underline{87.9}    &  70.2    &   \underline{82.7}  \\
% GPT-J-6B              &  78.4    &  \underline{88.0}    &  71.5     &  \underline{83.1}    \\
% SimCSE                &  85.1    &  \underline{89.7}    &  78.9    &  \underline{85.1}    \\
% SBERT*                &  87.8    &  \textbf{\underline{91.0}}    &  83.3    &  \textbf{\underline{87.0}}    \\ \hline
% \model~w/o LM                  &   -   &   86.7   &   -   &   81.5   \\
% % Best-two LMs                  &   90.0   &   91.9   &   85.3   &   88.0   \\
% \Xhline{3\arrayrulewidth}  
% \end{tabular}
% }
% \caption{Zero-shot performance on CoarseWSD-20.}
% \label{tab:wsd}
% \end{table}

% \begin{table}[!t]
% \centering
% \resizebox{7.5cm}{!}{%
% \begin{tabular}{lcccc}
% \Xhline{3\arrayrulewidth}  
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Accuracy}}             & \multicolumn{2}{c}{\textbf{F1}}       \\ \cline{2-5}
%   & \multicolumn{1}{l}{Orig.} & \multicolumn{1}{l}{\model} & \multicolumn{1}{l}{Orig.} & \multicolumn{1}{l}{\model} \\ \hline
% Random                &   41.3    &   -   &  36.7    &   -   \\
% BERT-L-1shot$^{\dagger}$*          &  77.6    &  -    &  71.2    &   -   \\
% BERT-L-3shot$^{\dagger}$*          &  89.3    &  -    &  85.2    &   -   \\ 
% RoBERTa-L-mnli*           &  80.4    &   \underline{83.0}  & 74.4    &  \underline{78.1}   \\
% BART-L-mnli*           &  80.2    &  \underline{82.4}    &  74.8   &  \underline{77.9}    \\
% GPT-Neo-1.3B          &  74.4    &  \underline{88.5}    &  68.4    & \underline{84.6}    \\
% GPT-Neo-2.7B          &  76.2    &  \underline{88.9}    &  70.2    &   \underline{85.2}  \\
% GPT-J-6B              &  78.4    &  \underline{88.5}    &  71.5     &  \underline{84.6}    \\
% OPT-30B \\
% SimCSE                &  85.1    &  \underline{89.7}    &  78.9    &  \underline{86.0}    \\
% SBERT*                &  87.8    &  \textbf{\underline{90.6}}    &  83.3    &  \textbf{\underline{87.5}}    \\ \hline
% \model~w/o LM                  &   -   &   87.7   &   -   &   83.8   \\
% % Best-two LMs                  &   90.0   &   91.9   &   85.3   &   88.0   \\
% \Xhline{3\arrayrulewidth}  
% \end{tabular}
% }
% \caption{Zero-shot performance on CoarseWSD-20.}
% \label{tab:wsd}
% \vspace{-0.3cm}
% \end{table}

\begin{table}[!t]
\centering
\resizebox{7.5cm}{!}{%
\begin{tabular}{lcccc}
\Xhline{3\arrayrulewidth}  
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Accuracy}}             & \multicolumn{2}{c}{\textbf{F1}}       \\ \cline{2-5}
   & \multicolumn{1}{l}{Orig.} & \multicolumn{1}{l}{\model} & \multicolumn{1}{l}{Orig.} & \multicolumn{1}{l}{\model} \\ \hline
Random                             &   41.3   &   -   &  36.7    &   -   \\
BERT-L-1shot$^{\dagger}$*          &  77.6    &  -    &  71.2    &   -   \\
BERT-L-3shot$^{\dagger}$*          &  89.3    &  -    &  85.2    &   -   \\ 
RoBERTa-L-mnli*       &  80.4    &  \underline{83.0}    &  74.4    &  \underline{78.1} \\
BART-L-mnli*          &  80.2    &  \underline{82.4}    &  74.8    &  \underline{77.9} \\
GPT-Neo-1.3B          &  84.7    &  \underline{88.4}    &  78.3    & \underline{84.6}  \\
GPT-Neo-2.7B          &  86.7    &  \underline{88.9}    &  81.5    & \underline{85.3}  \\
GPT-J-6B              &  84.1    &  \underline{88.5}    &  79.3    & \underline{84.8}  \\
OPT-30B               &  84.4    &  \underline{88.8}    &  80.4    & \underline{85.1}  \\
SimCSE                &  85.1    &  \underline{89.7}    &  78.9    &  \underline{86.0}    \\
SBERT*                &  87.8    &  \textbf{\underline{90.6}}    &  83.3    &  \textbf{\underline{87.5}}    \\ \hline
\model~w/o LM                  &   -   &   87.7   &   -   &   83.8   \\
% Best-two LMs                  &   90.0   &   91.9   &   85.3   &   88.0   \\
\Xhline{3\arrayrulewidth}  
\end{tabular}
}
\caption{Zero-shot performance on CoarseWSD-20.}
\label{tab:wsd}
\end{table}
\vspace{-.2cm}

